Mid-Training with Self-Generated Data Improves Reinforcement Learning in Language Models

The effectiveness of Reinforcement Learning (RL) in Large Language Models (LLMs) depends on the nature and diversity of the data used before and during RL. In particular, reasoning problems can often be approached in multiple ways that rely on different forms of reasoning, and exposure to only a limited range of such approaches in the training data may limit the effectiveness of RL. Motivated by this, we investigate using diverse self-generated data during mid-training as an intermediate step before RL training. Specifically, we adopt a bootstrapped data-generation framework guided by George Polya's problem-solving approaches for generating multiple variants of correct answers for each question in the training data, and then perform fine-tuning. We first provide a theoretical perspective on how mid-training on such data improves RL and explain how policy-gradient updates can incentivize combining multiple approaches. We then empirically demonstrate that RL-trained models initialized with our mid-training data achieve consistent improvements across various mathematical reasoning benchmarks and other OOD tasks like code generation and narrative reasoning. Overall, our investigative study shows that a language model learning multiple problem-solving approaches, through self-generated data helps subsequent RL.

==> theory/t1.tex <==
We analyze the mechanism by which diverse mid-training enables the emergence of novel behaviors during RL. Our analysis relies on the interaction between **Temperature Sampling** and the **Negative Gradient** updates inherent in RL algorithms like GRPO. We posit that diverse SFT creates a "latent reservoir" of strategies, and RL uses negative gradients to redistribute probability mass from failed attempts into this reservoir.

\paragraph{Preliminaries}
Let $\mathcal{Y}(x)$ be the space of all possible generated sequences for input $x$. We partition this space into three sets:
\begin{itemize}
    \item $\mathcal{S}_{\text{train}}$: The set of specific trajectories seen during SFT (the $K$ variations).
    \item $\mathcal{S}_{\text{latent}}$: The set of valid, high-quality trajectories that were \textit{not} explicitly seen, but are composed of learned heuristic patterns (the emergent behaviors).
    \item $\mathcal{S}_{\text{err}}$: The set of incorrect or nonsensical trajectories.
\end{itemize}

\begin{theorem}[Accessibility via Temperature Sampling]
Let $\pi_{\text{base}}$ be initialized on $K=1$ variation, and $\pi_{\text{div}}$ be initialized on $K \gg 1$ variations. Under temperature sampling with $\tau > 1$, the probability mass assigned to the latent valid set $\mathcal{S}_{\text{latent}}$ is lower-bounded by the diversity of the support:
\[
\mathbb{E}_{\pi_{\text{div}}^{(\tau)}} [\mathbb{1}_{y \in \mathcal{S}_{\text{latent}}}] > \mathbb{E}_{\pi_{\text{base}}^{(\tau)}} [\mathbb{1}_{y \in \mathcal{S}_{\text{latent}}}].
\]
\end{theorem}

\textit{Proof Sketch.} 
The softmax distribution with temperature $\tau$ is defined as $\pi^{(\tau)}(y|x) \propto \exp(z(y|x)/\tau)$. 
In $\pi_{\text{base}}$, the logits $z(y|x)$ are peaked around a single trajectory $y^*$. The "tail" of the distribution consists largely of random token perturbations which mostly fall into $\mathcal{S}_{\text{err}}$.
In $\pi_{\text{div}}$, the optimization objective maximizes logits for $K$ distinct heuristic paths. This creates a landscape with multiple local maxima. The region "between" these maxima (in the representation space) corresponds to hybrid strategies—e.g., combining the setup of Heuristic A with the derivation of Heuristic B. These hybrids constitute $\mathcal{S}_{\text{latent}}$.
Temperature sampling flattens the distribution. Because $\pi_{\text{div}}$ has high logits distributed across a wider semantic volume (the convex hull of the $K$ heuristics), the "flattened" probability mass flows into the interpolation region $\mathcal{S}_{\text{latent}}$. In contrast, flattening $\pi_{\text{base}}$ merely shifts mass into the vast, unstructured $\mathcal{S}_{\text{err}}$. \qed

\paragraph{The Role of Negative Gradients}
While temperature sampling provides \textit{access} to new behaviors, the RL update rule selects them. Recent work on efficient exploration (e.g., E3) highlights the critical role of **negative gradients**—signals derived from low-reward trajectories—in driving exploration via "Mass Spreading."

\begin{theorem}[Mass Spreading to Latent Strategies]
Consider an RL step where the model samples an incorrect trajectory $y_{\text{fail}} \in \mathcal{S}_{\text{err}}$ and receives a negative advantage $\hat{A} < 0$. The gradient update redistributes the probability mass removed from $y_{\text{fail}}$ to other trajectories $y'$ proportional to their current likelihood $\pi_t(y')$.
Specifically, if $\pi_t(y_{\text{fail}})$ decreases, the probability of a latent valid strategy $y_{\text{latent}}$ increases if and only if it has significant support in the current policy:
\[
\Delta \pi(y_{\text{latent}}) \propto -\pi_t(y_{\text{latent}}) \cdot \hat{A} \cdot \nabla \log \pi(y_{\text{fail}}) > 0.
\]
\end{theorem}

\textit{Proof.} 
The policy gradient update (simplified) approximates $\pi_{t+1}(y) \propto \pi_t(y) e^{\eta \hat{A}(y)}$.
When $y_{\text{fail}}$ is sampled with $\hat{A} < 0$, its probability decreases: $\pi_{t+1}(y_{\text{fail}}) < \pi_t(y_{\text{fail}})$.
Since $\sum_y \pi(y) = 1$, the probability mass lost by $y_{\text{fail}}$ must be redistributed to the remaining sequences. This redistribution is multiplicative; trajectories that already have non-trivial probability mass $\pi_t(y)$ receive the largest boost.
\begin{itemize}
    \item \textbf{Case Baseline ($\pi_{\text{base}}$):} The only sequence with high probability is the single training example $y^*$. Mass lost from errors is redistributed back to $y^*$. The model collapses to its initialization without exploring.
    \item \textbf{Case Diverse ($\pi_{\text{div}}$):} By Theorem 1, $\pi_t(y_{\text{latent}})$ is non-negligible due to the diverse support. When $y_{\text{fail}}$ is penalized, the "squeezed" probability mass spreads into $\mathcal{S}_{\text{latent}}$.
\end{itemize}
Thus, negative gradients act as a steering mechanism: they prune failures and, purely by the mechanics of the softmax normalization, force the policy to explore the pre-seeded valid strategies in $\mathcal{S}_{\text{latent}}$. This manifests as the emergence of new behaviors during RL. \qed
